Detecting Systematic Weaknesses in Vision Models along Predefined Human-Understandable Dimensions

Slice discovery methods (SDMs) are prominent algorithms for finding systematic weaknesses in DNNs. They identify top-k semantically coherent slices/subsets of data where a DNN-under-test has low performance. For being directly useful, slices should be aligned with human-understandable and relevant dimensions, which, for example, are defined by safety and domain experts as part of the operational design domain (ODD). While SDMs can be applied effectively on structured data, their application on image data is complicated by the lack of semantic metadata. To address these issues, we present an algorithm that combines foundation models for zero-shot image classification to generate semantic metadata with methods for combinatorial search to find systematic weaknesses in images. In contrast to existing approaches, ours identifies weak slices that are in line with pre-defined human-understandable dimensions. As the algorithm includes foundation models, its intermediate and final results may not always be exact. Therefore, we include an approach to address the impact of noisy metadata. We validate our algorithm on both synthetic and real-world datasets, demonstrating its ability to recover human-understandable systematic weaknesses. Furthermore, using our approach, we identify systematic weaknesses of multiple pre-trained and publicly available state-of-the-art computer vision DNNs.

==> images/table1_results.tex <==

\begin{tikzpicture}[every node/.style={draw, minimum width=1cm, minimum height=0.7cm}]

  \begin{table}[h]
    \setlength{\tabcolsep}{3pt}

    \centering
    \begin{tabular}{c|cccl}
    Slice No. & $\mathcal{|S|}$ & $FNR$ & \makecell{Avg. Perf. \\ Degra.} & Slice Description \\
        \hline

    $\mathcal{S}_1$     & 851	& 0.7086	& -0.0643 & \messagebubble{\makecell[l]{\textbf{age}: young \\
        \textbf{clothing-color}: dark-color}} \\
    \hline

    $\mathcal{S}_2$     & 338	& 0.7485	& -0.1042 & \messagebubble{\makecell[l]{\textbf{age}: young \\      
    \textbf{blurry}: true}} \\
    \hline   
    $\mathcal{S}_3$     & 368	& 0.731	    & -0.0867 & \messagebubble{\makecell[l]{\textbf{gender}: female \\
        \textbf{age}: young}} \\
    \hline

    % $\mathcal{S}_4$     & 59	& 0.2373	&-0.0789 & \messagebubble{\makecell[l]{\textbf{gender}: female \\
    %     \textbf{clothing-color}: bright-color}}\\
    % \hline

    % $\mathcal{S}_5$     & 23	& 0.3043	& -0.1460 & \messagebubble{\makecell[l]{\textbf{gender}: female \\
    %     \textbf{hair-color}: blond \\
    %     \textbf{clothing-color}: bright-color \\
    %     \textbf{construction-worker}: false}}\\
    \end{tabular}
    \caption{Quantitative analysis of the top-5 weak slices for the Panoptic-FCN model trained and evaluated on RailSem19 dataset. With the considered cut-off threshold, only 3 slices were found for this experiment.}
    \label{tab:appendix:railsem}
\end{table}
\end{tikzpicture}


==> sec/archive_4_experiment_setup.tex <==
% \section{Experiment Setup}
% \label{sec:experiment_setup}

% \textbf{Datasets:} We use four datasets in our experiments to test different black-box DNNs-under-test. First, as a proof-of-concept for our overall approach, we use the CelebA~\citep{liu2015faceattributes} dataset with a rich collection of 40 facial attributes (metadata) for $202\,599$ images of celebrity faces. We use the aligned PNG images provided by the authors, which are at a resolution of $178 \times 218$ pixels.
% Next, for the pedestrian detection tasks, we consider BDD100k~\citep{yu2020bdd100k}, Cityscapes~\citep{cordts2016cityscapes}, and RailSem19~\citep{Zendel_2019_CVPR_Workshops}. In these datasets, we focus only on the pedestrian class in the 2D-bounding box and semantic segmentation tasks. For BDD100k, we consider the predefined validation set of 10k samples of resolution $1280 \times 720$, while in Cityscapes and RailSem19, due to their smaller dataset sizes, we use the entire train and val sets containing 3475 and 8500 samples with image resolutions $2048 \times 1024$ and $1920 \times 1080$ respectively.
% % \ma{Comparison to SOTA approaches, namely PromptAttack \cite{Metzen_2023_ICCV} and CounTEX \cite{kim2023grounding}, is provided using above CelebA and ``Animals with Attributes 2'' (AwA2) dataset~\cite{xian2018zero}, where for the latter we focus on the ``hippopotamus'' class.}
% %In addition, to compare against SOTA approaches, we use results from CelebA and Animals with Attributes2 (AwA2) dataset~\cite{xian2018zero} which contains 50 animal classes and 85 attributes. However, for our benchmarking experiment, we focus primarily on the "hippopotamus" class. 

% \textbf{Models (DNNs-under-test):} We evaluate four black-box models for ODD aligned systematic weaknesses. For the first experiment, we consider the publicly available ViT-B-16~\citep{dosovitskiy2020image} model pre-trained on ImageNet21k~\citep{ridnik2021imagenet} from the python library timm, \mar{\cite{timm_github}}.\footnote{\url{https://github.com/huggingface/pytorch-image-models}}
% % Although this model is trained to classify~11k classes, we focus on the hierarchy level 1 semantic classes as proposed in \cite{ridnik2021imagenet}.
% % As we only focus on data subset~\textit{"n00007846"}, all images do in fact contain "person". 
% Second, we use the pre-trained publicly available Faster R-CNN~\citep{ren2015faster} object detector with ConvNeXt-T~\citep{liu2022convnet} backbone. The model weights are available on the BDD100k model Zoo.\footnote{\url{https://github.com/SysCV/bdd100k-models/tree/main/det}} Third, for the Cityscapes dataset, we use a pre-trained SETR PUP~\citep{zheng2021rethinking} semantic segmentation model. The model weights are available on the mmsegmentation codebase, \mar{\cite{mmseg2020}}.\footnote{\url{https://github.com/open-mmlab/mmsegmentation}}
% Finally, from the railway domain, we use a PanopticFCN~\citep{li2021fully} model, which has been trained by an industrial partner on a large proprietary dataset also including  RailSem19~\citep{Zendel_2019_CVPR_Workshops}. We consider this as a complete black box and have no details on the concrete training. 
% For the autonomous datasets, the black-box model performance per object (i.e., pedestrian) is measured by the intersection-over-union (IoU).

% \textbf{Parameters} of CLIP and SliceLine:
% For the metadata generation, we use a pre-trained CLIP~\citep{radford2021learning} with image encoder (ViT-L/14~\citep{dosovitskiy2020image}).
% For SliceLine, we use a python implementation\footnote{\url{https://github.com/DataDome/sliceline}} and choose default $\alpha$ and $\sigma$ values of $0.95$ and $n/100$ \sg{move this to the appendix} where $n$ defines the size of the structured data as proposed in \citep{sagadeeva2021sliceline}. We run the experiments for a depth level of 5 and present the top-5 weak slices. 
% To foster reproducibility, we will provide the overall code and the prompts used for metadata generation with CLIP.
% %\sg{code and prompts will be provided}



